AutoGluon-Tabular: Robust and Accurate AutoML for Structured Data

We introduce AutoGluon-Tabular, an open-source AutoML framework that requires only a single line of Python to train highly accurate machine learning models on an unprocessed tabular dataset such as a CSV file. Unlike existing AutoML frameworks that primarily focus on model/hyperparameter selection, AutoGluon-Tabular succeeds by ensembling multiple models and stacking them in multiple layers. Experiments reveal that our multi-layer combination of many models offers better use of allocated training time than seeking out the best. A second contribution is an extensive evaluation of public and commercial AutoML platforms including TPOT, H2O, AutoWEKA, auto-sklearn, AutoGluon, and Google AutoML Tables. Tests on a suite of 50 classification and regression tasks from Kaggle and the OpenML AutoML Benchmark reveal that AutoGluon is faster, more robust, and much more accurate. We find that AutoGluon often even outperforms the best-in-hindsight combination of all of its competitors. In two popular Kaggle competitions, AutoGluon beat 99% of the participating data scientists after merely 4h of training on the raw data.

==> OGopenml_core_1h_pairwise_autogluon_1h.tex <==
\begin{tabular}{lccccccc}
\toprule
   \textbf{System} &  \textbf{$>$ AutoGluon (1h)} &  \textbf{$<$ AutoGluon (1h)} &  \textbf{Failures} &  \textbf{Best} &  \textbf{Rank} &  \textbf{Test Loss Rescaled} & \textbf{Time (m)} \\
\midrule
    AutoGluon (1h) &                            0 &                            0 &                  0 &             19 &         1.5455 &                       0.0474 &                57 \\
   GCP-Tables (1h) &                            6 &                           20 &                 13 &              5 &         2.8182 &                       0.2010 &                90 \\
   H2O AutoML (1h) &                            8 &                           30 &                  1 &              5 &         3.1818 &                       0.1914 &                58 \\
 auto-sklearn (1h) &                            8 &                           26 &                  5 &              4 &         3.7273 &                       0.2176 &                60 \\
         TPOT (1h) &                            5 &                           30 &                  4 &              4 &         4.0909 &                       0.2900 &                67 \\
    Auto-WEKA (1h) &                            4 &                           31 &                  4 &              2 &         5.6364 &                       0.9383 &                62 \\
\bottomrule
\end{tabular}


==> OGopenml_core_4h_pairwise_autogluon_4h.tex <==
\begin{tabular}{lccccccc}
\toprule
   \textbf{System} &  \textbf{$>$ AutoGluon (4h)} &  \textbf{$<$ AutoGluon (4h)} &  \textbf{Failures} &  \textbf{Best} &  \textbf{Rank} &  \textbf{Test Loss Rescaled} & \textbf{Time (m)} \\
\midrule
    AutoGluon (4h) &                            0 &                            0 &                  1 &             23 &         1.8438 &                       0.1385 &               201 \\
   H2O AutoML (4h) &                            4 &                           26 &                  8 &              2 &         3.1250 &                       0.2447 &               220 \\
         TPOT (4h) &                            6 &                           27 &                  5 &              5 &         3.3750 &                       0.2034 &               235 \\
   GCP-Tables (4h) &                            5 &                           20 &                 14 &              4 &         3.7500 &                       0.3336 &               195 \\
 auto-sklearn (4h) &                            6 &                           27 &                  6 &              3 &         3.8125 &                       0.3197 &               240 \\
    Auto-WEKA (4h) &                            4 &                           28 &                  6 &              1 &         5.0938 &                       0.8001 &               244 \\
\bottomrule
\end{tabular}


==> ablationtable.tex <==
\begin{tabular}{cc}
\toprule
   \textbf{Variant of AutoGluon} &  \textbf{Average Test Loss}  \\
\midrule
    \emph{Full System}  &   0.2554 \\
  \emph{NoRepeat} & 0.2562 \\
  \emph{NoStack} & 0.2670 \\
  \emph{NoBag} & 0.2728 \\
  \emph{NoNetwork} & 0.2808 \\
  \emph{NoEnsemble} & \todo{?} \\
\bottomrule
\end{tabular}



==> openml_ablation_1h_pairwise_autogluon_1h.tex <==
\begin{tabular}{lcccccc}
\toprule
\textbf{Framework} &  \textbf{Wins} &  \textbf{Losses} &  \textbf{Champion} &  \textbf{Avg. Rank} &  \textbf{Avg. Rescaled Loss} & \textbf{Avg. Time (min)} \\
\midrule
         AutoGluon &              0 &                0 &                 10 &              2.3462 &                       0.2734 &                       55 \\
          NoRepeat &             17 &               20 &                 13 &              2.4872 &                       0.3200 &                       44 \\
      NoMultiStack &             14 &               24 &                  8 &              3.0128 &                       0.5240 &                       53 \\
             NoBag &             11 &               28 &                  5 &              3.3462 &                       0.6260 &                       16 \\
         NoNetwork &              9 &               30 &                  1 &              3.8077 &                       0.7654 &                       11 \\
\bottomrule
\end{tabular}


==> openml_ablation_4h_pairwise_autogluon_4h.tex <==
\begin{tabular}{lcccccc}
\toprule
\textbf{Framework} &  \textbf{Wins} &  \textbf{Losses} &  \textbf{Champion} &  \textbf{Avg. Rank} &  \textbf{Avg. Rescaled Loss} & \textbf{Avg. Time (min)} \\
\midrule
         AutoGluon &              0 &                0 &                 17 &              1.9324 &                       0.1660 &                      192 \\
          NoRepeat &             17 &               20 &                 12 &              2.1216 &                       0.2199 &                      114 \\
      NoMultiStack &              7 &               28 &                  6 &              2.8514 &                       0.5237 &                      173 \\
             NoBag &              5 &               33 &                  3 &              3.9054 &                       0.7199 &                       27 \\
         NoNetwork &              5 &               33 &                  0 &              4.1892 &                       0.8171 &                       16 \\
\bottomrule
\end{tabular}


==> openml_ablation_combined_pairwise_autogluon_1h.tex <==
\begin{tabular}{lcccccc}
\toprule
\textbf{Framework} &  \textbf{Wins} &  \textbf{Losses} &  \textbf{Champion} &  \textbf{Avg. Rank} &  \textbf{Avg. Rescaled Loss} & \textbf{Avg. Time (min)} \\
\midrule
    AutoGluon (4h) &             30 &                5 &                 15 &              2.6757 &                       0.1416 &                      192 \\
     NoRepeat (4h) &             25 &               13 &                 11 &              3.3919 &                       0.2106 &                      114 \\
    AutoGluon (1h) &              0 &                0 &                  2 &              4.6351 &                       0.3323 &                       55 \\
 NoMultiStack (4h) &             16 &               21 &                  3 &              4.6622 &                       0.4361 &                      173 \\
     NoRepeat (1h) &             17 &               20 &                  2 &              4.9595 &                       0.3600 &                       43 \\
 NoMultiStack (1h) &             14 &               24 &                  2 &              6.1351 &                       0.5868 &                       53 \\
        NoBag (1h) &             11 &               28 &                  1 &              6.6351 &                       0.6513 &                       15 \\
        NoBag (4h) &             10 &               29 &                  1 &              7.0405 &                       0.6605 &                       27 \\
    NoNetwork (1h) &              9 &               30 &                  0 &              7.4189 &                       0.7475 &                       10 \\
    NoNetwork (4h) &              9 &               30 &                  0 &              7.4459 &                       0.7431 &                       16 \\
\bottomrule
\end{tabular}


==> openml_accuracy_1h_openml_alllosses_1h.tex <==
\begin{tabular}{lccccccc}
\toprule
  \textbf{Dataset} & \textbf{Auto-WEKA} & \textbf{auto-sklearn} &   \textbf{TPOT} & \textbf{H2O AutoML} & \textbf{GCP-Tables} & \textbf{AutoPilot} & \textbf{AutoGluon} \\
\midrule
        APSFailure &              0.007 &                 0.006 &           0.008 &               0.004 &               0.005 &              0.005 &     \textbf{0.004} \\
          Airlines &                 x  &                 0.331 &           0.356 &               0.378 &      \textbf{0.327} &              0.332 &              0.344 \\
            Albert &              0.379 &                 0.314 &           0.348 &               0.336 &               0.310 &              0.352 &     \textbf{0.307} \\
 Amazon\_employee\_a &              0.052 &        \textbf{0.050} &           0.052 &               0.050 &               0.054 &              0.054 &              0.051 \\
        Australian &     \textbf{0.130} &                    x  &  \textbf{0.130} &      \textbf{0.130} &                  x  &                 x  &     \textbf{0.130} \\
         Covertype &              0.357 &                 0.033 &           0.243 &               0.115 &               0.066 &                 x  &     \textbf{0.023} \\
            Dionis &     \textbf{0.114} &                    x  &           0.458 &                  x  &                  x  &                 x  &              0.163 \\
     Fashion-MNIST &              0.150 &                 0.120 &           0.232 &               0.106 &               0.100 &                 x  &     \textbf{0.097} \\
            Helena &              0.723 &                 0.670 &           0.676 &               0.628 &                  x  &              0.633 &     \textbf{0.628} \\
            Jannis &              0.355 &                    x  &           0.290 &               0.273 &               0.277 &              0.281 &     \textbf{0.271} \\
 KDDCup09\_appetenc &              0.019 &        \textbf{0.017} &  \textbf{0.017} &               0.024 &      \textbf{0.017} &     \textbf{0.017} &     \textbf{0.017} \\
         MiniBooNE &              0.095 &                 0.061 &           0.064 &               0.056 &               0.055 &              0.059 &     \textbf{0.053} \\
            Robert &                 x  &                 0.536 &              x  &      \textbf{0.502} &                  x  &                 x  &              0.507 \\
           Shuttle &       \textbf{0.0} &                 0.000 &           0.000 &               0.000 &                  x  &              0.000 &              0.000 \\
           Volkert &              0.379 &                 0.328 &           0.353 &               0.301 &               0.301 &              0.300 &     \textbf{0.265} \\
             adult &              0.144 &                 0.125 &           0.124 &               0.131 &               0.124 &              0.128 &     \textbf{0.123} \\
    bank-marketing &              0.092 &                 0.090 &           0.091 &               0.092 &               0.090 &              0.094 &     \textbf{0.089} \\
 blood-transfusion &               0.24 &                  0.24 &  \textbf{0.213} &               0.226 &                  x  &                 x  &               0.24 \\
               car &              0.208 &          \textbf{0.0} &    \textbf{0.0} &        \textbf{0.0} &        \textbf{0.0} &              0.005 &       \textbf{0.0} \\
         christine &              0.317 &                 0.265 &           0.267 &               0.263 &                  x  &              0.261 &     \textbf{0.249} \\
            cnae-9 &              0.148 &        \textbf{0.018} &  \textbf{0.018} &      \textbf{0.018} &                  x  &                 x  &              0.046 \\
         connect-4 &              0.292 &                 0.176 &           0.140 &               0.133 &      \textbf{0.119} &              0.135 &              0.128 \\
          credit-g &                0.2 &                    x  &   \textbf{0.19} &                0.22 &                  x  &                 x  &               0.21 \\
           dilbert &              0.027 &                 0.015 &           0.069 &               0.022 &                  x  &              0.021 &     \textbf{0.008} \\
            fabert &              0.396 &                 0.266 &           0.308 &               0.275 &               0.294 &              0.276 &     \textbf{0.265} \\
        guiellermo &                 x  &                 0.182 &             0.4 &               0.151 &                  x  &                 x  &     \textbf{0.149} \\
             higgs &              0.395 &                 0.268 &           0.272 &               0.277 &      \textbf{0.258} &              0.285 &              0.264 \\
           jasmine &              0.183 &                 0.170 &           0.187 &               0.183 &      \textbf{0.167} &              0.214 &              0.173 \\
 jungle\_chess\_2pcs &              0.254 &                 0.084 &           0.081 &               0.090 &      \textbf{0.001} &              0.045 &              0.009 \\
               kc1 &              0.142 &                 0.151 &           0.132 &               0.137 &               0.127 &                 x  &     \textbf{0.123} \\
          kr-vs-kp &              0.009 &        \textbf{0.003} &              x  &               0.006 &               0.006 &              0.006 &              0.006 \\
     mfeat-factors &     \textbf{0.015} &                  0.03 &           0.035 &               0.025 &                0.02 &              0.035 &               0.02 \\
             nomao &              0.022 &        \textbf{0.017} &           0.019 &               0.024 &               0.026 &              0.029 &              0.020 \\
       numerai28.6 &     \textbf{0.479} &                 0.488 &              x  &               0.494 &               0.481 &              0.488 &              0.489 \\
           phoneme &              0.077 &                 0.109 &           0.097 &               0.094 &               0.086 &              0.099 &     \textbf{0.075} \\
          riccardo &                 x  &                    x  &              x  &      \textbf{0.002} &                  x  &                 x  &     \textbf{0.002} \\
           segment &              0.012 &        \textbf{0.008} &           0.012 &      \textbf{0.008} &      \textbf{0.008} &              0.012 &     \textbf{0.008} \\
           sylvine &              0.076 &                 0.064 &           0.048 &               0.058 &               0.058 &              0.062 &     \textbf{0.042} \\
           vehicle &              0.141 &                 0.164 &  \textbf{0.129} &               0.141 &                  x  &                 x  &              0.152 \\
\bottomrule
\end{tabular}


==> openml_core10fold_1h_pairwise_autogluon_1h.tex <==
\begin{tabular}{lccccccc}
\toprule
\textbf{Framework} &  \textbf{Wins} &  \textbf{Losses} &  \textbf{Failures} &  \textbf{Champion} &  \textbf{Avg. Rank} &  \textbf{Avg. Rescaled Loss} & \textbf{Avg. Time (min)} \\
\midrule
         AutoGluon &              0 &                0 &                  0 &                 26 &              1.3929 &                       0.0324 &                       56 \\
        H2O AutoML &             11 &               26 &                  2 &                  9 &              2.2143 &                       0.0836 &                       58 \\
      auto-sklearn &              6 &               28 &                  5 &                  3 &              3.0357 &                       0.1587 &                       60 \\
              TPOT &              3 &               31 &                  5 &                  1 &              3.3929 &                       0.2128 &                       72 \\
         Auto-WEKA &              1 &               33 &                  5 &                  0 &              4.9643 &                       0.9913 &                       61 \\
\bottomrule
\end{tabular}


==> openml_orig10fold_1h_pairwise_autogluon_1h.tex <==
\begin{tabular}{lccccccc}
\toprule
\textbf{Framework} &  \textbf{Wins} &  \textbf{Losses} &  \textbf{Failures} &  \textbf{Champion} &  \textbf{Avg. Rank} &  \textbf{Avg. Rescaled Loss} & \textbf{Avg. Time (min)} \\
\midrule
         AutoGluon &              0 &                0 &                  0 &                 22 &              1.7500 &                       0.0335 &                       55 \\
        H2O AutoML &              9 &               25 &                  1 &                  2 &              3.0833 &                       0.0581 &                       58 \\
    H2O AutoML (O) &             10 &               24 &                  1 &                  5 &              3.3750 &                       0.0690 &                       55 \\
      auto-sklearn &              5 &               26 &                  4 &                  1 &              4.3750 &                       0.1083 &                       60 \\
  auto-sklearn (O) &              4 &               30 &                  1 &                  1 &              4.8333 &                       0.1096 &                       60 \\
              TPOT &              3 &               28 &                  4 &                  1 &              5.2500 &                       0.1502 &                       71 \\
          TPOT (O) &              4 &               30 &                  1 &                  2 &              5.5833 &                       0.2016 &                       65 \\
     Auto-WEKA (O) &              1 &               30 &                  4 &                  0 &              8.3333 &                       0.7770 &                       62 \\
         Auto-WEKA &              1 &               31 &                  3 &                  0 &              8.4167 &                       0.7471 &                       60 \\
\bottomrule
\end{tabular}

